Finite difference method on flat surfaces with a flat unitary vector bundle

We establish an asymptotic relation between the spectrum of the discrete Laplacian associated to discretizations of a half-translation surface with a flat unitary vector bundle and the spectrum of the Friedrichs extension of the Laplacian with von Neumann boundary conditions. As an interesting byproduct of our study, we obtain Harnack-type estimates on "almost harmonic" discrete functions, defined on the graphs, which approximate a given surface. The results of this paper will be later used to relate the asymptotic expansion of the number of spanning trees, spanning forests and weighted cycle-rooted spanning forests on the discretizations to the corresponding zeta-regularized determinants.

==> Files/packages.tex <==
\usepackage{times}

\usepackage[utf8]{inputenc}
\usepackage{commath}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{cite}
\usepackage{natbib}
\usepackage{bigints}
\usepackage{comment}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage{ifthen}

\usepackage{pst-node}
\usepackage{tikz-cd} 
\usepackage{fancyhdr}



%\usepackage{showkeys}
\allowdisplaybreaks[4]

\numberwithin{equation}{section}


==> Files/paddings.tex <==
\usepackage[%
    left=1in,%
    right=1in,%
    top=1.1in,%
    bottom=0.8in,%
    paperheight=11in,%
    paperwidth=8.5in%
]{geometry}

==> Files/theorem.tex <==
\theoremstyle{definition}
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem*{prop*}{Proposition}
\newtheorem{defn}[thm]{Definition}
\newtheorem*{thm*}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{exmp}[thm]{Example}
\newtheorem{asump}[thm]{Assumption}
\newtheorem{notat}[thm]{Notation}
\newtheorem{const}[thm]{Construction}

\newcommand{\thmexpl}[1] {\noindent{#1}}

\newcounter{tmp}

==> Files/title.tex <==
\title{Relative spectral theory for surfaces with cusps II. \\
The curvature theorem and Deligne pairing.} 

\author
{Siarhei Finski
}

\date{}

